Multi-Agent Reinforcement Learning in Stochastic Networked Systems

We study multi-agent reinforcement learning (MARL) in a stochastic network of agents. The objective is to find localized policies that maximize the (discounted) global reward. In general, scalability is a challenge in this setting because the size of the global state/action space can be exponential in the number of agents. Scalable algorithms are only known in cases where dependencies are static, fixed and local, e.g., between neighbors in a fixed, time-invariant underlying graph. In this work, we propose a Scalable Actor Critic framework that applies in settings where the dependencies can be non-local and stochastic, and provide a finite-time error bound that shows how the convergence rate depends on the speed of information spread in the network. Additionally, as a byproduct of our analysis, we obtain novel finite-time convergence results for a general stochastic approximation scheme and for temporal difference learning with state aggregation, which apply beyond the setting of MARL in networked systems.

==> submission_history.tex <==
%

Prior to this submission, a version of this paper was submitted to the 34th Conference on Learning Theory (COLT 21). The main concerns from the reviewers were regarding the presentation. This was the only concern raised by the meta-reviewer. Specifically, the reviewers found it difficult to understand our networked MARL setting and interpret the $\mu$-decay condition. In preparing the paper for this submission we have improved the readability of our paper by adding extra explanations and discussion about each setting in sections 4.0, 4.1, and 4.2. We also added discussion to emphasize the importance of each set of our results in Sections 2, 3, and 4.1. We further simplified some of the complex mathematical expressions in the body, pushing the complexity to the appendix, so as to facilitate understanding. Finally, we reformulated the statement of Theorem 4.5 in order to make the result more interpretable, as suggested by the previous reviewers.
